Independent Learning in Performative Markov Potential Games

Performative Reinforcement Learning (PRL) refers to a scenario in which the deployed policy changes the reward and transition dynamics of the underlying environment. In this work, we study multi-agent PRL by incorporating performative effects into Markov Potential Games (MPGs). We introduce the notion of a performatively stable equilibrium (PSE) and show that it always exists under a reasonable sensitivity assumption. We then provide convergence results for state-of-the-art algorithms used to solve MPGs. Specifically, we show that independent policy gradient ascent (IPGA) and independent natural policy gradient (INPG) converge to an approximate PSE in the best-iterate sense, with an additional term that accounts for the performative effects. Furthermore, we show that INPG asymptotically converges to a PSE in the last-iterate sense. As the performative effects vanish, we recover the convergence rates from prior work. For a special case of our game, we provide finite-time last-iterate convergence results for a repeated retraining approach, in which agents independently optimize a surrogate objective. We conduct extensive experiments to validate our theoretical findings.

==> 5_algorithms.tex <==
% !TEX root =  main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Algorithms}

For independent learning, we use the following PGA method, introduced by \citet{IndepPolicyGrad_Ding}. \\

Algorithm~\ref{alg:PGA} is the conceptual algorithm, assuming exact estimations $\Bar{Q}_{i,t}^t$. (infinite sample setting).

\begin{algorithm}
\caption{Independent Policy Gradient Ascent}
\label{alg:PGA}
\begin{algorithmic}[1]
    \State{\textbf{Input}:} Step size $\eta$
    \State{\textbf{Init.:}} for all $i \in \mathcal{N}, a_i \in \mathcal{A}_i , s \in S$, let $\pi^t_i(a_i | s ) = 1/|\mathcal{A}_i| $.
    \For{$t=1$ to $T$}
        \For{$i=1$ to $n$ (simultaneously)}
            \State Define $\overline{Q}_{i,t}^{t}(s, a_i) = \sum_{a_{-i}} \pi_{-i}(a_{-i} \mid s) \cdot Q_{i, t}^{t}(s, a_i, a_{-i})$
            \State $\displaystyle
                \pi^{t+1}_i(\cdot | s) = \argmax_{\pi(\cdot | s ) \in \Delta(\mathcal{A}_i)} \Big\{ \big\langle \pi_i(\cdot | s), \overline{Q}_{i, t}^t(s, \cdot) \big\rangle_{\mathcal{A}_i} - \frac{1}{2\eta} \cdot \lVert \pi_i(\cdot | s) - \pi_i^t(\cdot|s) \rVert^2\Big\}
            $
        \EndFor
    \EndFor
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:PGA_finite} is for the finite sample case.

\begin{algorithm}
\caption{Policy Gradient Ascent - Finite Samples}
\label{alg:PGA_finite}
\begin{algorithmic}[1]
    \State{\textbf{Input}:} Step size $\eta$, $K = \#\textit{trajectories per time step}$
    \State{\textbf{Init.:}} for all $i \in \mathcal{N}, a_i \in \mathcal{A}_i , s \in S$, let $\pi^t_i(a_i | s ) = 1/|\mathcal{A}_i| $.
    \\
    \For{$t=1$ to $T$}
        \State{\textcolor{gray}{\texttt{\# }Phase $1$: Data collection}} 
        \\ 
        \For{$k=1$ to $K$}
            \State{For each agent $i \in \mathcal{N}$, sample $h_i, h'_i$ from a geometric distribution with parameter $(1-\gamma)$}
            \State{draw initial state $\overline{s}^{0} \sim \rho$}
            \State{Continuing from $s^{0}$, for $H = max_i(h_i + h'_i)$ steps, using $\pi^t$, we generate the state-joint-action-reward trajectory $\overline{s}^{0}, \overline{a}^{0}, \overline{r}^{0}, \overline{s}^{1}, \overline{a}^{1}, \overline{r}^{1}, \dots, \overline{s}^{H}, \overline{a}^{H}, \overline{r}^{H}$} w.r.t. the underlying shared MDP $M(\pi^{t})$
        \State{Define for every agent $i \in \mathcal{N}$:}
            $\displaystyle \;
            \overline{s}_i^k := \Bar{s}^{h_i},
            \quad
            \overline{a}_i^k := \overline{a}_i^{h_i},
            \quad
                R^k_{i} := \sum_{h = h_i}^{h_i + h'_i - 1} \overline{r}^{h}_i
            $
        \EndFor
        \State{\textcolor{gray}{\texttt{\# }Phase 2: Policy Update}}
        \For{$i=1$ to $n$ (simultaneously)}
            % \State Define $\overline{Q}_{i,t}^{t}(s, a_i) = \sum_{a_{-i}} \pi_{-i}(a_{-i} \mid s) \cdot Q_{i, t}^{t}(s, a_i, a_{-i})$. \\
            \State Compute %\widehat{Q}^t_{i}$ via 
            $\displaystyle
                \widehat{Q}^t_i(\cdot,\cdot) \quad  \approx \argmin_{ \lVert \widehat{Q}_{i,t}^t(\cdot, \cdot) \rVert_2 \leq \frac{\sqrt{|\mathcal{S}| \cdot |\mathcal{A}|}}{1-\gamma}} \quad \sum_{k=1}^K \Big(R^k_{i,t} - \widehat{Q}_{i,t}^t(\overline{s}_i^k,\overline{a}_i^k) \Big)^2$.
            \\
            %\State Compute $\widehat{\omega}_{i, t}^t$ via
            %$\displaystyle
            %    \widehat{\omega}^t_{i,t} \approx \argmin_{ \lVert \omega_i \rVert \leq W} \sum_{k=1}^K \Big(R^k_{i,t} - \langle \phi_i(s^{h_i}, a_i^{h_i}), \omega^t_{i,t} \rangle \Big)^2
            %$
            %\State $\widehat{Q}^t_i(s, \cdot) = \langle \phi_i(s, \cdot), \widehat{\omega}^t_{i,t} \rangle$ and player's $i$ policy for $s \in \mathcal{S}$
            \State Define $\Delta_{\xi}(\mathcal{A}_i) := \{ (1-\xi) \pi_i(\cdot \mid s) + \frac{\xi}{|\mathcal{A}_i|}, \forall \pi_i(\cdot \mid s) \}$ ($\xi$-greedy exploration)
            \State For any $s \in \mathcal{S}$ (Lazy updates):
            \State $\displaystyle
                \pi^{t+1}_i(\cdot | s) = \argmax_{\pi(\cdot | s ) \in \Delta_\xi(\mathcal{A}_i)} \Big\{ \big\langle \pi_i(\cdot | s), \widehat{Q}_{i, t}^t(s, \cdot) \big\rangle_{\mathcal{A}_i} - \frac{1}{2\eta} \cdot \lVert \pi_i(\cdot | s) - \pi_i^t(\cdot|s) \rVert_2^2\Big\}.
            $
        \EndFor
    \EndFor
\end{algorithmic}
\end{algorithm}

